Perceptual Gradient Networks

Many applications of deep learning for image generation use perceptual losses for either training or fine-tuning of the generator networks. The use of perceptual loss however incurs repeated forward-backward passes in a large image classification network as well as a considerable memory overhead required to store the activations of this network. It is therefore desirable or sometimes even critical to get rid of these overheads. In this work, we propose a way to train generator networks using approximations of perceptual loss that are computed without forward-backward passes. Instead, we use a simpler perceptual gradient network that directly synthesizes the gradient field of a perceptual loss. We introduce the concept of proxy targets, which stabilize the predicted gradient, meaning that learning with it does not lead to divergence or oscillations. In addition, our method allows interpretation of the predicted gradient, providing insight into the internals of perceptual loss and suggesting potential ways to improve it in future work.

==> 6_conclusion.tex <==
\section{Conclusion}
\label{sect:conclusion}

We have presented perceptual gradient networks (PGNs) that allow to approximate the gradient of the perceptual loss with a simple feedforward pass, while being less time- and memory-intensive. For a number of diverse applications, we have shown that training with PGNs achieves a similar effect on the resulting images as training with the original perceptual loss. We have also shown how proxy targets, while being noisy, highlight important detail in images, which might pave way for an improved and more efficient perceptual loss.
